Distribution-Aware Calibration for Object Detection with Noisy Bounding Boxes

Large-scale well-annotated datasets are of great importance for training an effective object detector. However, obtaining accurate bounding box annotations is laborious and demanding. Unfortunately, the resultant noisy bounding boxes could cause corrupt supervision signals and thus diminish detection performance. Motivated by the observation that the real ground-truth is usually situated in the aggregation region of the proposals assigned to a noisy ground-truth, we propose DIStribution-aware CalibratiOn (DISCO) to model the spatial distribution of proposals for calibrating supervision signals. In DISCO, spatial distribution modeling is performed to statistically extract the potential locations of objects. Based on the modeled distribution, three distribution-aware techniques, i.e., distribution-aware proposal augmentation (DA-Aug), distribution-aware box refinement (DA-Ref), and distribution-aware confidence estimation (DA-Est), are developed to improve classification, localization, and interpretability, respectively. Extensive experiments on large-scale noisy image datasets (i.e., Pascal VOC and MS-COCO) demonstrate that DISCO can achieve state-of-the-art detection performance, especially at high noise levels. Code is available at https://github.com/Correr-Zhou/DISCO.

==> tables/execution.tex <==
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{1pt}
  \renewcommand{\arraystretch}{1.6}
  \resizebox{0.4\linewidth}{!}{
    \setlength{\tabcolsep}{3mm}{
\begin{tabular}{c|c}
\specialrule{0.15em}{0pt}{0pt}
Execution Number of DISCO & $\text{AP}_{50}$ \bigstrut\\
\hline
\hline
1     & 68.1 \bigstrut[t]\\
2     & \textbf{68.7} \\
3     & 67.9 \bigstrut[b]\\
\specialrule{0.15em}{0pt}{0pt}
\end{tabular}

}}    
     \caption{
     \textbf{Ablation studies of the execution number of DISCO.}
     Our execution strategy can achieve superior performance.
     }
      
    \label{tab:execution}
    \vspace{-5mm}
\end{table}


==> tables/original.tex <==
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{1pt}
  \renewcommand{\arraystretch}{1.6}
    \resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{2.4mm}{
    \begin{tabular}{l|c|cccccc}
    \hline
    \multirow{2}[4]{*}{Method} & VOC   & \multicolumn{6}{c}{COCO} \bigstrut\\
\cline{2-8}          & $\text{AP}_{50}$ & $\text{AP}$ & $\text{AP}_{50}$ & $\text{AP}_{75}$ & $\text{AP}_\text{S}$ & $\text{AP}_\text{M}$ & $\text{AP}_\text{L}$ \bigstrut\\
    \hline
    \hline
    OA-MIL & 77.1  & 37.0  & 57.9  & 40.3  & 21.8  & 40.6  & 47.6 \bigstrut[t]\\
    DISCO (Ours) & \textbf{78.0} & \textbf{38.0} & \textbf{57.9}  & \textbf{41.9} & \textbf{21.9} & \textbf{41.4}  & \textbf{48.5} \bigstrut[b]\\
    \hline
    \end{tabular}%
    }}
     \caption{
     \textbf{Experimental results on the original VOC and COCO.}
     Unlike OA-MIL, Our DISCO can still provide performance improvement even without manually introducing noise.
     }
    \vspace{-2mm}
    \label{tab:original}
\end{table}

